TS-Net: Combining modality specific and common features for multimodal patch matching

Multimodal patch matching addresses the problem of finding the correspondences between image patches from two different modalities, e.g. RGB vs sketch or RGB vs near-infrared. The comparison of patches of different modalities can be done by discovering the information common to both modalities (Siamese like approaches) or the modality-specific information (Pseudo-Siamese like approaches). We observed that none of these two scenarios is optimal. This motivates us to propose a three-stream architecture, dubbed as TS-Net, combining the benefits of the two. In addition, we show that adding extra constraints in the intermediate layers of such networks further boosts the performance. Experimentations on three multimodal datasets show significant performance gains in comparison with Siamese and Pseudo-Siamese networks.

==> tex_network_architecture__1_.tex <==
\begin{figure*}[tb]
\centering
\includegraphics[width=0.85\textwidth]{images_network_architecture.png}
\caption{The detailed architectures of (a) standard Siamese networks (b) Siamese networks with the proposed additional loss on the feature towers  (c) the proposed TS-Net network with additional losses on the feature extraction tower and on the metric network. The numbers on each rectangle indicate the output size of this layer.}
\label{fig:network_architecture}
\end{figure*}

\section{The Proposed Three-Stream Network}
\label{sec:network_architecture}

As explained before, the proposed architecture for multimodal patch matching, denoted as the TS-Net architecture, is intended to combine the advantages of both Siamese and Pseudo-Siamese networks. The overall architecture of TS-Net  is given Fig. \ref{fig:network_architecture}(c). Each sub-network has 2 main parts: two feature extraction towers and a metric learning module. In the case of the Siamese network, the parameters of the feature extraction towers are shared, while for Pseudo-Siamese networks they are distinct.  TS-Net takes a pair of patches as input, one from each modality, and predicts independently in each sub-network whether they are similar or not. Finally, the outputs of each sub-network are combined by an additional fully connected (FC) layer to produce the final prediction. 
In the next paragraphs, the different components of TS-Net are described and commented.

\vspace{.8em}\noindent \textbf{Feature extraction network.} Each tower is based on convolutional and pooling layers to hierarchically extract high-level information from the input patches. We use max-pooling layers to reduce the dimensions of the feature maps by a factor of 2. At the end of the tower, we use a bottleneck (fully connected) layer to produce a compact output vector with 128 dimensions. Inspired from \cite{han2015matchnet}, we use $Relu$ activation as a non-linear activation function.

\vspace{.8em}\noindent \textbf{Tower Fusion.} We observed in our experiments that 
subtracting the layers produced better performance than concatenating them, as in the original MatchNet. So the output of the feature extraction tower are element-wise subtracted before they are fed to the metric network.

\vspace{.8em}\noindent \textbf{Metric network.} The metric learning part of the network consists of three fully connected layers. It takes a vector of 128 dimensions and produces a vector of dimension two, suitable for binary classification.

\vspace{.8em}\noindent \textbf{Losses.}  We treat patch matching as a binary classification problem, as we observed it performs better (also observed by \cite{tian2017l2}) than learning a similarity function. Therefore, Siamese and Pseudo-Siamese parts of TS-Net are trained with binary cross-entropy loss functions.

One contribution of this paper is to introduce additional constraints, at the feature level, by  means of a contrastive loss \cite{chopra2005learning} enforcing the features coming from the two feature towers to be close to each other if the pair is positive. This will enable the features of positive pairs to be in the hypersphere and the features of the negative pairs to be outside the hypersphere.

The fusion of Siamese and Pseudo-Siamese networks is done by introducing an additional cross-entropy loss on the top of the two. 

More formally, let $(x_1, x_2)$ be the input pair of patches and $y$ the class label. $y=1$ means the pair is positive (similar patches), $y=0$ means the pair is negative (different patches). We denote by $L_{en}$ and $L_{con}$  the cross-entropy and the contrastive loss, with:\\ (a) $L_{en} = y \log(\hat{y}) + (1-y)\log(1-\hat{y})$ where $\hat{y}$ is output of the \textit{Softmax} layer, and \\ (b) 
$L_{con} = y \frac{2}{Q}D^2 + (1-y)2Qe^{\frac{-2.77}{Q}D}$
%\label{equ:lambda}
%\end{equation}
where $D$ is the Euclidean distance between features. Q is the margin to be optimized.
The overall loss function is then given by:\\ $
L = L_{tsnet_{en}} + L_{siam_{en}} +   L_{pseudo_{en}} + \lambda L_{siam_{con}} +   \beta L_{pseudo_{con}}$, with $\lambda$ and $\beta $ two cross-validated parameters in $[0,1]$. 

In multimodal settings, it is not always guaranteed that the two modalities can be projected into the same subspace.  In practice, we observed that optimal performance is obtained for $\lambda$ and $\beta$  set to $10^{-2}$ (values obtained by cross validating the parameters on the validation set).

\vspace{.8em}\noindent \textbf{Implementation details.} We initialize the weights of each convolutional layer  using the Xavier initialization and all the FC layers with a truncated normal distribution ($stddev=0.005$ and $mean=0$, $bias=0.1$). While the original MatchNet is trained with plain stochastic gradient descent, we found that training with 0.95 momentum produce equal or better performance. We train the network with $lr=10^{-3}$ with L2 regularization of $10^{-3}$ with neither dropout nor $batchnorm$. $Q$ is optimized experimentally on VeDAI validation set and set to be 50 for the other two datasets. During training, we observe that the $\lambda$ and $\beta$ parameters should be carefully set and the best performance we obtain is for $\lambda = 10^{-2}, \beta = 10^{-4}$ or $\beta = 10^{-2}$ on CUHK and NIR Scene (cross validation experiments). We use batch size of 32 and train with at least 150 epochs. All the experimentations are done using Tensorflow 1.4 with NVIDIA P100 or K80 GPU. Patches are normalized to have zero mean and unit standard deviation for each modality.
